VerilogReader: LLM-Aided Hardware Test Generation

Test generation has been a critical and labor-intensive process in hardware design verification. Recently, the emergence of Large Language Model (LLM) with their advanced understanding and inference capabilities, has introduced a novel approach. In this work, we investigate the integration of LLM into the Coverage Directed Test Generation (CDG) process, where the LLM functions as a Verilog Reader. It accurately grasps the code logic, thereby generating stimuli that can reach unexplored code branches. We compare our framework with random testing, using our self-designed Verilog benchmark suite. Experiments demonstrate that our framework outperforms random testing on designs within the LLM's comprehension scope. Our work also proposes prompt engineering optimizations to augment LLM's understanding scope and accuracy.

==> tables/covergroup.tex <==
\begin{table*}[t]
\center
\caption{Coverage Closure Target in Fuzzing}
\begin{tabular*}{\linewidth}{p{2.5cm}p{7.5cm}p{5cm}p{2cm}}
\hline\\[-2.9mm]\hline
Coverage & Description & Pseudo Code & Point Count\\
\hline
Line Coverage &  Number of Verilog basic blocks executed during testing. & - & 733\\

Branch Coverage & Number of Verilog branch trace points executed during testing. & - & 839\\
\hline

Router Covergroup1 
& 
\thead[lp{7cm}]{Possible states of requests (enabled or disabled) from five input ports to a single output port arbiter. Each output port has one associated covergroup. }
& 
\thead[l]{for output port x: \textit{cross} \\ req$_{n\_to\_x}$,  req$_{e\_to\_x}$, req$_{s\_to\_x}$, \\ req$_{w\_to\_x}$, req$_{p\_to\_x}$} 
& 
800\\ 

Router Covergroup2 
&
\thead[lp{7cm}]{Possible states of request sending directions(free or directed towards NWESP) from five input ports. }
&
\thead[l]{\textit{cross} \\ input-req$_{n}$,  input-req$_{e}$, input-req$_{s}$, \\ input-req$_{w}$, input-req$_{p}$} 
& 
7776\\

Router Covergroup3 
& 
\thead[lp{7cm}]{Possible states of five output ports' granting(free or granted to NWESP input port). Some state combinations are impossible(\eg{multi output ports granting to one input port}). }
& 
\thead[l]{\textit{cross} \\ output-gnt$_{n}$,  output-gnt$_{e}$, output-gnt$_{s}$, \\ output-gnt$_{w}$, output-gnt$_{p}$} 
& 
1546\\
\hline



Mesh Covergroup1 
&
\thead[lp{7cm}]{Possible states of buffers usage for selected local input ports during data send request in $3\times3$ Mesh. We divide 16-size buffer into 6 states.}
& 
\thead[l]{\textit{cross} \\ buffer-P$_{(0,0)}$,  buffer-P$_{(0,1)}$, \\ buffer-P$_{(1,0)}$, buffer-P$_{(1,1)}$}
&
1296
\\

Mesh Covergroup2
&
\thead[lp{7cm}]{Possible states of buffers usage of five input ports of the center router during data send request in $3\times3$ Mesh. We divide 16-size buffer into 6 states.}
& 
\thead[l]{\textit{cross} \\ buffer-N$_{(1,1)}$,  buffer-E$_{(1,1)}$, buffer-S$_{(1,1)}$, \\ buffer-W$_{(1,1)}$, buffer-P$_{(1,1)}$}
&
486
\\

Mesh Covergroup3
& 
\thead[lp{7cm}]{Possible states of request sending destinations(free or sent to other 8 routers) from selected local input ports in $3\times3$ Mesh. }
& 
\thead[l]{\textit{cross} \\ input-req$_{(0,0)}$,  input-req$_{(0,1)}$, \\ input-req$_{(1,0)}$, input-req$_{(1,1)}$}
& 
6561\\

\hline\\[-2.9mm]\hline
\end{tabular*}
\label{tab:coverage_description}
\end{table*}

==> tables/exp-result.tex <==
\begin{table*}[h]
\centering
\caption{Test generation methods effectiveness comparison.}
% \tabcolsep=1cm
\renewcommand\arraystretch{1.2}
\begin{tabular}{cc|p{1.1cm}<{\centering}p{1.1cm}<{\centering}p{1.3cm}<{\centering}p{1.3cm}<{\centering}p{1.4cm}<{\centering}|p{1.4cm}<{\centering}p{1.3cm}<{\centering}p{1.3cm}<{\centering}} 
\hline\\[-3.4mm]\hline

\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Result}} & \multicolumn{5}{c}{\textbf{Router}} & \multicolumn{3}{c}{\textbf{Mesh Network}}\\ 
\cline{3-10}
 & & Line & Branch & Covergroup1 & Covergroup2 & Covergroup3 & Covergroup1 & Covergroup2 & Covergroup3 \\ 
 
\hline
\multirow{2}{*}{Random} & \textit{Time (h)} & 120 & 120 & 120 & 120 & 0.55  & 120 & 120 & \textbf{0.33} \\
 & \textit{Cov (\%)} & 96.7 & 94.8 & 97.3 & 98.6 & \textit{max}  & 99.8 & 89.7 & \textit{\textbf{max}}\\
 
\hline
\multirow{2}{*}{CRV} & \textit{Time (h)} & 120 & 120 &  120 &  23.6 &  \textbf{0.17} & - & - & - \\
 & \textit{Cov (\%)} & 97.3 & 95.2 & 98.8 & \textit{max} & \textit{\textbf{max}} & - & - & - \\
 
\hline
\multirow{2}{*}{Fuzz} & \textit{Time (h)} & \textbf{2.6} & \textbf{2.4} & \textbf{3.3} & \textbf{10.8} & 1.0  & \textbf{9.2} & \textbf{6.8} & 5.1\\
 & \textit{Cov (\%)} & \textit{\textbf{max}} & \textit{\textbf{max}} & \textit{\textbf{max}} & \textit{\textbf{max}}  & \textit{max} & \textit{\textbf{max}} & \textit{\textbf{max}} & \textit{max}\\
 
\hline\\[-3.4mm]\hline
\end{tabular}
\label{tab:exp_result}
\end{table*}

==> tables/noc-smoke-test.tex <==
\begin{table}[b]
\centering
\begin{tabular}{|c|c|l|}
\hline
\textbf{DUT} & \textbf{No.} & \textbf{\centering{Description \textit{(\#x means at clock cycle x)}}} \\
\hline
\multirow{7}{*}{Router} 
 & 1 & W to E, 1 packet \\
 & 2 & N to E, 1 packet \\
 & 3 & W\_\#1 + N\_\#1 to E, 1 packet \\
 & 4 & W\_\#1 + N\_\#2 to E, 1 packet \\
 & 5 & W\_\#1 + N\_\#25 + S\_\#33 to E, 1 packet \\
 & 6 & W\_\#1 + N\_\#33 + S\_\#33 to E, 1 packet \\
 & 7 & ... \\
\hline
\multirow{7}{1cm}{\centering Mesh \\ Network \\ (2$*$2)} 
 & 1 & R$_0$ to R$_2$ , 1 packet \\
 & 2 & R$_1$ to R$_2$ , 1 packet \\
 & 3 & R$_0$\_\#0 + R$_1$\_\#0 to R$_3$, 1 packet \\
 & 4 & R$_0$\_\#0 + R$_1$\_\#1 to R$_3$, 1 packet \\
 & 5 & R$_0$\_\#0 + R$_1$\_\#0 + R$_2$\_\#0 to R$_3$, 1 packet \\
 & 6 & R$_0$\_\#0 + R$_1$\_\#24 + R$_2$\_\#24 to R$_3$, 1 packet \\
 & 7 & ... \\
\hline
\end{tabular}
\caption{Human-written NoC test cases.}
\label{tab:noc-test-case}
\end{table}
